Text-aware Speech Separation for Multi-talker Keyword Spotting

For noisy environments, ensuring the robustness of keyword spotting (KWS) systems is essential. While much research has focused on noisy KWS, less attention has been paid to multi-talker mixed speech scenarios. Unlike the usual cocktail party problem where multi-talker speech is separated using speaker clues, the key challenge here is to extract the target speech for KWS based on text clues. To address it, this paper proposes a novel Text-aware Permutation Determinization Training method for multi-talker KWS with a clue-based Speech Separation front-end (TPDT-SS). Our research highlights the critical role of SS front-ends and shows that incorporating keyword-specific clues into these models can greatly enhance the effectiveness. TPDT-SS shows remarkable success in addressing permutation problems in mixed keyword speech, thereby greatly boosting the performance of the backend. Additionally, fine-tuning our system on unseen mixed speech results in further performance improvement.

==> content/results.backup.tex <==
% FRR -> recall
\begin{table*}[htbp]
    \label{tab:fusion_methods}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c c  c c  c  c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Snips2mix}} & \multicolumn{2}{c}{\textbf{Libri2mix}} & \multicolumn{1}{c}{\textbf{KWS}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6}
        &   STOI & SI-SNR & STOI & SI-SNR & chn1 \\
        \midrule
        text only(TSKiM) & 85.96 & 9.71 & 84.52 & 9.52 & 7.20\% \\
        audio only & 86.02 & 9.87 & 84.73 & 9.65 & 10.37\% \\
        \midrule 
        append & 86.15 & 9.95 & 84.58 & 9.55 & 8.40\% \\
        concat & \textbf{86.29} & \textbf{9.95} & \textbf{84.86} & \textbf{9.63} & \textbf{8.27\%} \\
        concat + avg-pooling & 86.22 & 9.90 & 84.76 & 9.53 & 9.40\% \\
        FiLM ~\cite{perez2018film} & 84.23 & 9.30 & 84.16 & 9.31 & 8.70\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Results on different audio-text information fusion methods with TSKiM-10.}
\end{table*}


\begin{table*}[htbp]
    \label{tab:separation}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c c c  c  c c  c c c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\bm{$\mathcal{L}_{PIT}$}} & \multirow{2}{*}{\bm{$\mathcal{L}_{k}$}} & \multicolumn{2}{c}{\textbf{Snips2mix}} & \multicolumn{2}{c}{\textbf{Libri2mix}} & \multicolumn{2}{c}{\textbf{KWS}} \\
        \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        &  & &   STOI & SI-SNR & STOI & SI-SNR & max & chn1 \\
        \midrule
        Skim & \ding{51} &  \ding{56} &86.04 & 9.93 & \textbf{84.93} & \textbf{9.74} & 17.20\% & 58.23\% \\ 
        TSkim & \ding{56} &  \ding{51} \\ 
        TSkim & \ding{51} & \ding{56} & 85.91 & 9.78 & 84.62 & 9.59 &  20.30\% & 59.87\% \\
        \midrule 
        TSkim & \ding{51} & \ding{51} & 85.96 & 9.71 & 84.52 & 9.52 & 7.80\% & 7.20\% \\
        TSkim-10 & \ding{51} & \ding{51} & 86.29 & 9.95 & 84.86 & 9.63 & 7.93\% & 8.27\% \\
        TSkim-20 & \ding{51} & \ding{51} & 86.21 & 9.76 & 84.62 & 9.52 & 9.17\% & 7.30\% \\
        TSkim-50 & \ding{51} & \ding{51} & \textbf{86.33} & \textbf{10.00} & 84.76 & 9.66 & 5.10\% & \textbf{4.73\%} \\
        TSkim-100 & \ding{51} & \ding{51} & 86.15 & 9.91 & 84.76 & 9.59 & 9.77\% & 9.13\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance of SS models trained on both \textbf{Snips2mix} and \textbf{Libri2mix}.}
\end{table*}

\begin{table*}[htbp]
    \label{tab:kws_ft}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c  c   c  c  c  c  c}
        \toprule
        \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Non-FT}} & \multicolumn{1}{c}{\textbf{FT on SKiM}} & \multicolumn{1}{c}{\textbf{FT on TSKiM-50}}  & \multicolumn{1}{c}{\textbf{FT on SKiM + 2000}} & \multicolumn{1}{c}{\textbf{FT on TSKiM-50 + 2000}} & \multicolumn{1}{c}{\textbf{FT on corr. data + 2000}} \\
        \midrule
        Skim & 17.20\% & 17.90\% & 8.63\% & 19.27\% & 9.23\% & 19.27\% \\ 
        TSkim & 7.20\% & 8.30\% & 3.07\% & 6.63\% & 3.37\% & 3.50\% \\
        TSkim-10 & 8.27\% & 8.53\% & 4.57\% & 6.87\% & 4.00\% & 3.87\% \\
        TSkim-20 & 7.30\% & 6.67\% & 3.53\% & 6.53\% & 4.17\% & 3.97\% \\
        TSkim-50 & 4.73\% & 6.60\% & 3.23\% & 6.10\% & \textbf{2.43\%} & \textbf{2.43\%} \\
        TSkim-100 & 9.13\% & 8.43\% & 5.57\% & 7.23\% & 5.43\% & 4.87\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{KWS finetune using audios from separation models chn1, FRR/0.5 FA.}
\end{table*}

\begin{table*}[htbp]
    \label{tab:kws_on_mix}
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{ c c c}
        \toprule
        \multicolumn{1}{c}{\textbf{Training Data}} & \multicolumn{1}{c}{\textbf{Test Data}} & \multicolumn{1}{c} {\textbf{FRR/0.5 FA}} \\
        \midrule
        Snips & Clean & 2.57\% \\
        Snips & Mix & 80.77\% \\
        Snips2Mix + Libri2Mix & Mix & 32.93\% \\
        Snips2Mix + Libri2Mix + 2000 & Mix & 26.93\% \\
        Snips + Snips2Mix + Libri2Mix & Mix & 17.17\% \\
        Snips + Snips2Mix + Libri2Mix + 2000 & Mix & 23.90\% \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance of KWS models trained on \textbf{Snips2mix}.}
\end{table*}



